Formation of super-Earths and mini-Neptunes from rings of planetesimals

The solar system planetary architecture has been proposed to be consistent with the terrestrial and giant planets forming from material rings at ~1 au and ~5 au, respectively. Here, we show that super-Earths and mini-Neptunes may share a similar formation pathway. In our simulations conducted with a disk alpha-viscosity of 4e-3, super-Earths accrete from rings of rocky material in the inner disk, growing predominantly via planetesimal accretion. Mini-Neptunes primarily originate from rings located beyond the water snowline, forming via pebble accretion. Our simulations broadly match the period-ratio distribution, the intra-system size uniformity, and the planet multiplicity distribution of exoplanets. The radius valley constrains the typical total mass available for rocky planet formation to be less than 3-6 Earth masses. Our results predict that planets at ~1 au in systems with close-in super-Earths and mini-Neptunes are predominantly water-rich. Though relatively uncommon, at ~1% level, such systems might also host rocky Earth-sized planets in the habitable zone that underwent late giant impacts, akin to the Moon-forming event.

==> introduction_backup.tex <==

Super-Earths and mini-Neptunes, planets of sizes ranging from 1 to 4 Earth radii, orbit at least 30\% of sun-like stars in our galaxy~\citep{Howard+2010, Borucki+2010, Batalha+2013, Fressin+2013, Fabrycky+2014}. Their size distribution is bimodal, with peaks at approximately 1.4 and 2.4 Earth radii and a gap around 1.8 Earth radii, known as the ``exoplanet radius valley'' \citep{Fulton+2017, Fulton+2018}. This feature suggests a composition dichotomy: planets of about 1.4 Earth radii are likely dominated by silicate compositions, while those with sizes around 2.4 Earth radii may have significant volatile content in their cores or primordial H-He rich atmospheres~\citep{Kuchner03, Fortney+2007, Adams+2008, Rogers+2010, Owen+2017, Zeng+2019, Venturini+2020, Izidoro+2022}. Yet, the origins of these planets remain a subject of strong debate.

Several formation and post-formation mechanisms have been proposed to explain the exoplanet radius valley, including atmospheric photoevaporation \citep{Lopez+2013, Owen+2019}, core-powered mass loss \citep{Ginzburg+2018, Gupta+2022}, impact-induced mass loss \citep{Liu+2015, Inamdar+2016, Biersteker+2019, Kegerreis+2020, Matsumoto+2021, Chance+2022}, hydrogen sequestration into a magma ocean \citep{Kite2020}, and efficient hydrodynamic water mass loss \citep{Burn+2024}. Combining the atmospheric mass loss mechanisms with the formation models, the origin of the radius valley has been investigated. Population synthesis models invoking planetesimal accretion as the primary mechanism of planetary growth show that rocky and icy/water-rich planets can grow and migrate to close-in orbits \citep{Jin+2014, Jin+2018, Burn+2024}. However, the compositional dichotomy of planets produced within this model does not form a clear radius valley because this model produces too many water-rich planets. To address this inconsistency between the model and observations, \citet{Burn+2024} propose that photoevaporation of a water-rich atmosphere could further erode planetary atmospheres, leading to significant water loss if the upper atmosphere and the deep envelope of these planets are efficiently mixed. 

Contrary to the planetesimal accretion model, \citet{Venturini+2020} shows that a compositional dichotomy naturally appears in the close-in orbit and forms the deep radius valley when planets grow via pebble accretion. Using N-body simulations, \citet{Izidoro+2022} confirm that a compositional dichotomy arises among close-in planets within the pebble accretion framework. 

The above studies successfully form the radius valley in close-in planets. However, the planetesimal accretion scenario requires small planetesimals as 300 meters in radius to form planets in outer orbit  \citep{Burn+2024}, and the pebble accretion scenario needs unrealistically high pebble flux, about 10 times greater than canonical dust-to-gas ratios to form rocky planets inside water ice line \citep{Izidoro+2022}. Also, these formation models implicitly assume that planetesimals form everywhere in the protoplanetary disk and form a continuous distribution in the planetesimal disk. 
%In \citet{Burn+2024}, where planets form via planetesimal accretion, the initial planetesimal distribution is given by an exponential scaling law. \citet{Izidoro+2022}, based on the pebble accretion scenario, distributes seed planets uniformly in the protoplanetary disk. 
The current planetesimal formation models do not support such initial distribution of planetesimals.
%and seed planets. 

%However, it remains unclear whether such a complete mixing can realistically occur or if their difficulty in explaining the radius valley is a consequence of their formation model. Most planet population synthesis models by \cite{Burn+2024} (and references therein) assume that planets form purely via planetesimal accretion and planetesimals to be approximately 300 meters in radius. Yet, planetesimal formation models indicate that typical planetesimal sizes are much larger than 300 meters, typically $\sim$100~km.  While impact-induced fragmentation could be a mechanism to produce smaller planetesimals, excessive fragmentation poses a problem, as it can inhibit planet formation rather than support it \cite{Kaufmann+2023}. These caveats limit the applicability of these models for gaining insights into observations. 

%However, they also find that forming super-Earths and mini-Neptunes in the same planetary system via pebble accretion requires an unrealistically high pebble flux, about 10 times greater than canonical dust-to-gas ratios. This limitation arises because the accretion efficiency of small, rocky pebbles inside the water ice line is too low to allow for the rapid formation of rocky super-Earths, indicating a need for exceptionally high pebble fluxes that may not be realistic.

%Planet formation starts from dust coagulation, drift, fragmentation, and turbulent mixing in a young protoplanetary disk \citep{Birnstiel+2024}. 

% -- kilometer-sized building blocks of planets -- 
Planetesimals are thought to form under specific conditions in regions of the disk where the local dust-to-gas ratio is sufficiently high for dust to concentrate into clumps and gravitationally collapse \citep{Youdin2005, Johansen+2007, Johansen+2009, Bai+2010}. Pressure bumps in the gaseous disk, often associated with condensation fronts~\citep{Bitsch+2015a, Hyodo+2019, Hyodo+2021, Charnoz+2021} or transitions in disk viscosity~\citep{Masset+06, Desch+2015, Flock+2017}, provide ideal sites for planetesimal formation~\citep{Johansen+2007, Taki+16}. In pressure bumps, the radial drift-velocity of dust grains, caused by gas drag, is reduced or ceased~\citep{Adachi+1976}, leading to an increase in the local dust-to-gas ratio, potentially allowing planetesimals to form~\citep{Drazkowska+2017, Lichtenberg+2021, Carrera+22}.

Recent planet formation models propose that the building blocks of solar system planets formed at pressure bumps near the silicate sublimation line and the water snowline \citep{Izidoro+2021b, Morbidelli+2021}. As the disk's temperature evolved and the pressure bumps' location shifted, planetesimals were formed in ring-like distributions. The formation of the solar system's terrestrial planets is consistent with a ring of planetesimals extending from about 0.7 to 1.5 au, containing approximately 2 $M_\oplus$ of material~\citep{Hansen+2009, Walsh+2016}. The gas giant planets are thought to have originated from a second ring of planetesimals beyond the snowline~\citep{Brasser+2020, Lichtenberg+2021, Izidoro+2021b, Morbidelli+2021, Lau+2022, Lau+2024}, where more solid material was available for accretion, and pebble accretion was likely more efficient, facilitating the rapid formation of solid planetary cores becoming gas giants \citep{Lambrechts+2014}. Therefore, the silicate sublimation line and the water snowline are currently envisioned for the formation location of terrestrial and giant planets in the solar system~\citep{Drazkowska+2018, Lichtenberg+2021, Izidoro+2021b, Morbidelli+2021}.

Asteroid populations and dynamical evolution models support the view that the solar system formed from rings of planetesimals rather than from a wide and continuous disk~\citep{Deienno+2024, Brasser2024}. Recent models show that the asteroid belt (located between 2 and 3.2 AU) likely formed either empty or with very low mass (a few times its current mass of $5\times10^{-4}M_{\oplus}$) \citep{Mothe-diniz+2003, Demeo+2014}. In the classical framework of solar system formation, where planetesimals are thought to have been continuously distributed across the solar system, the asteroid belt's primordial total mass is expected to be a few Earth masses \citep{Hayashi+1981, Wetherill1996}. Within this scenario, one should expect to exist a significantly higher number of Vesta-sized objects in the asteroid belt than what is currently observed \citep{Deienno+2024}.

In this study, we develop a planet formation model coupled with post-formation processes to demonstrate that super-Earths and mini-Neptunes may have formed at two distinct regions of their natal gaseous disk, similar to what is currently envisioned for the terrestrial and giant planets in the solar system. In Sec.~\ref{sec: Methods}, we describe our formation model, which combines the planetesimal accretion and pebble accretion based on the formation of two planetesimal rings. We show our numerical results in Sec.~\ref{sec: Result}. We compare our numerical results with the California Kepler Survey (CKS). Section~\ref{sec: Discussion} discusses our results and numerical model. %We summarize this study in Sec.~\ref{sec: Summary}.

%-- specifically, impact-induced mass loss and atmospheric photoevaporation -- 


